A unified approach to shape and topological sensitivity analysis of discretized optimal design problems

We introduce a unified sensitivity concept for shape and topological perturbations and perform the sensitivity analysis for a discretized PDE-constrained design optimization problem in two space dimensions. We assume that the design is represented by a piecewise linear and globally continuous level set function on a fixed finite element mesh and relate perturbations of the level set function to perturbations of the shape or topology of the corresponding design. We illustrate the sensitivity analysis for a problem that is constrained by a reaction-diffusion equation and draw connections between our discrete sensitivities and the well-established continuous concepts of shape and topological derivatives. Finally, we verify our sensitivities and illustrate their application in a level-set-based design optimization algorithm where no distinction between shape and topological updates has to be made.

==> my_commands.tex <==
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{proposition}[theorem]{Proposition}
%%%%%
\newcommand{\ie}{\textit{i.e.}\,}
\newcommand{\eg}{\textit{e.g.}\,}
\newcommand{\R}{\mathbb R}
%\newcommand{\C}{\mathbb C}
\newcommand{\eps}{\varepsilon}
\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\rred}{\color{red}}
\newcommand{\gray}[1]{{\color{gray}{#1}}}
\newcommand{\blue}[1]{{\color{blue}{#1}}}
\newcommand{\bblue}{\color{blue}}
\newcommand{\olive}{\color{olive}}
\newcommand{\black}{\color{black}}
\newcommand{\green}{\color{green}}
%%%%%
\newcommand{\di}{\mathrm{i}}
\newcommand{\dd}{\;\mathrm{d} }
\newcommand{\ddx}{\;\mathrm{d} {\mathbf x}}
\newcommand{\ddsx}{\;\mathrm{d} s_{\mathbf x}}
\newcommand{\vect}[1]{{\mathbf #1}}
%%%%%
\newcommand{\um}[1]{\unit[#1]{m}}
\newcommand{\Nm}[1]{\unitfrac[#1]{N}{m^3}}
\newcommand{\Nmm}[1]{\unitfrac[#1]{N}{m^2}}
%\newcommand{\um}[1]{#1}
%\newcommand{\Nm}[1]{#1}
%\newcommand{\Nmm}[1]{#1}
%%%%%
\newcommand{\indA}{\alpha}
\newcommand{\indB}{\beta}
\newcommand{\indC}{\gamma}
\newcommand{\indD}{\varphi}
\newcommand{\indE}{\varkappa}
\newcommand{\indF}{\xi}
\newcommand{\indG}{\psi}
\newcommand{\indH}{\varsigma}
%%%%% finite element 
\newcommand{\mesh}{\mathcal{T}} 
\newcommand{\pos}{{\mathbf x}}
\newcommand{\levelset}{\phi}
\newcommand{\setIk}{I_{\pos_k}}
\newcommand{\setJl}{J_{\tau_l}}
\newcommand{\setRk}{R_{\pos_k}}
\newcommand{\detJl}{\left|{\textup{\text{det}}}J_l\right|}
%%%%
\newcommand{\phiVec}{{\pmb\phi}}
\newcommand{\targetU}{\hat u}
\newcommand{\targetUvec}{\hat {\mathbf u}}
%%%%%
\newcommand{\objectiveFunction}{g}
\newcommand{\phiObjectiveFunction}{J}
\newcommand{\redObjectiveFunction}{\mathfrak g} %reduced to Omega objective function
\newcommand{\redPhiObjectiveFunction}{\mathcal J} %reduced to phi objective function
%%%%%
\newcommand{\Tplus}{T^{-\rightarrow+}_{k,\varepsilon}}
\newcommand{\Tminus}{T^{+\rightarrow-}_{k,\varepsilon}}
\renewcommand{\S}{S_{k,\varepsilon}}
\newcommand{\SComplex}{ S_{k,ih}}
\newcommand{\TplusComplex}{T^{-\rightarrow+}_{k, ih}}
\newcommand{\TminusComplex}{T^{+\rightarrow-}_{k,ih}}
\newcommand{\SHyper}{S_{k,h_1E_1+h_2E_2+0E_1E_2}}
\newcommand{\TplusHyper}{T^{-\rightarrow+}_{k,h_1E_1+h_2E_2+0E_1E_2}}
\newcommand{\TminusHyper}{T^{+\rightarrow-}_{k,h_1E_1+h_2E_2+0E_1E_2}}
%
\newcommand{\operator}{O} 
\newcommand{\discreteOperator}{O_{k,\varepsilon}} % 
\newcommand{\setTplus}{\mathfrak T^+}
\newcommand{\setTminus}{\mathfrak T^-}
\newcommand{\setS}{\mathfrak S}
\newcommand{\elementAreaDerivativeShape}{da^S_l}
\newcommand{\finiteElementSpace}{S_h^1(D)} % better S_h^1(\mesh) ? 
\newcommand{\rhsF}{\hat {f}}
\newcommand{\rhsFvec}{\hat {\mathbf f}}
\newcommand{\symmDiff}{\triangle}
\newcommand{\defC}{c_t}	
\newcommand{\Mref}[1]{\Cref{#1}}
\newcommand{\changeArea}{\delta_{k,\eps} a}
\newcommand{\topshapeDerivative}{{topological-shape }}
\newcommand{\mylim}{\underset{t \searrow 0}{\mbox{lim }}}
\newcommand{\BL}{\dot{BL}(\mathbb R^2)}
